Nonparametric Bayesian Classification

A Bayesian approach to the classification problem is proposed in which random partitions play a central role. It is argued that the partitioning approach has the capacity to take advantage of a variety of large-scale spatial structures, if they are present in the unknown regression function $f_0$. An idealized one-dimensional problem is considered in detail. The proposed nonparametric prior uses random split points to partition the unit interval into a random number of pieces. This prior is found to provide a consistent estimate of the regression function in the $\L^p$ topology, for any $1 \leq p < \infty$, and for arbitrary measurable $f_0:[0,1] \to [0,1]$. A Markov chain Monte Carlo (MCMC) implementation is outlined and analyzed. Simulation experiments are conducted to show that the proposed estimate compares favorably with a variety of conventional estimators. A striking resemblance between the posterior mean estimate and the bagged CART estimate is noted and discussed. For higher dimensions, a generalized prior is introduced which employs a random Voronoi partition of the covariate-space. The resulting estimate displays promise on a two-dimensional problem, and extends with a minimum of additional computational effort to arbitrary metric spaces.

==> ch1.tex <==
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}

\newcommand{\Cvec}{\mathbf{C}}
\newcommand{\cvec}{\mathbf{c}}

In this thesis we consider the problem of binary regression and the
related classification (discrimination) problem. Specifically, the
data we consider is a list of pairs $(X_1,Y_1), (X_2,Y_2), \dots, \breakpt
(X_n, Y_n)$. Each $X$ is an explanatory variable through which attempt
to ``predict'' the corresponding label $Y$ which is either $0$ or
$1$. We model these pairs as being drawn $\iid$ from an unknown
distribution $F_0$ which we decompose as:
\[
dF_0\left( (x,y)
\right)=\big[f_0(x)\1{y=1}+(1-f_0(x))\1{y=0}\big]
\mu(dx)\eta(dy).
\]
Here $\1{}$ signifies the indicator function; $f_0(x)$ represents the
probability that $Y=1$ given that $X=x$; $\mu$ is the marginal
distribution of $X$ over the space $\X$; and $\eta$ is counting
measure on the set $\Y=\{0,1\}$. This decomposition is unique except
that, technically, $f_0$ is only determined $\mu$-a.e by $F_0$. 

In binary regression, our goal is to estimate $f_0$ (say in an $\cL^2$
or $\cL^1$ sense). For classification, we are only concerned with
being able to predict the most likely value of $Y$, equivalently we
are concerned with estimating the set $\{x:
f_0(x)>\frac{1}{2}\}$. There are a great many ways to proceed, as
evidenced by the vast literature on these subjects. Some references
are given in \secref{@@}.

\section{An Example}

To get started, let us consider the specific case in which
$\X=[0,1]$ and $\mu$ is uniform measure. Further, I choose a specific
$f_0$ which is piecewise continuous with two constant regions and a
smooth transition region. I take $f_0(x)$ to be:
\[
\1{0 \leq x < \frac{1}{6}} 0.6 + \1{\frac{1}{6} \leq x \leq
\frac{1}{2}} 0.4 + \1{\frac{1}{2} < x \leq 1} \Psi(x)
\]

where $\Psi(x)$ is :

\[
\Psi(x)=\frac{\phi_\sigma(x-\frac{1}{2})}{\phi_\sigma(x-\frac{1}{2})+\phi_\sigma(x-1)}
\]

and where $\phi_\sigma$ is the p.d.f. of a normal with mean 0 and
standard deviation $\sigma=0.25$.

\begin{figure}
\noindent
\begin{minipage}[t]{\linewidth}
  \centering%\epsfig{figure=figs/prob1plot.ps,height=5cm,angle=-90}
  \caption[]{$f(x)$}
\end{minipage}
\end{figure}

\section{A Nonparametric Prior on Regression Functions}

In the Bayesian approach, we specify our uncertainty about $F_0$, or,
equivalently, $f_0$ by specifying a probability distribution on
them. Ideally, we want this distras
randomly chosen.To specify our prior, I explain how to choose an $f$ at random
from it. First, choose $K$, the number of split points, where:
\[
P(K=k)=(1-\alpha)\alpha^k \quad \textrm{for $k=0 \dots \infty$}
\] 

That is, $K+1$ (the number of intervals) is geometric with parameter
$1-\alpha$.

Now, conditional on $K=k$, choose $C_1, C_2, \dots C_k$ \iid from
$U(0,1)$. Let $C_{(i)}$ (for $i=1 \dots k$) be the $i'th$ ordered value
of the $C$'s. This produces $k+1$ intervals:
\[
I_1=\{0 \leq x < C_{(1)}\}, I_2=\{C_{(1)} \leq x < C_{(2)}\}, \dots,
I_{k+1}=\{C_{(k)} \leq x \leq 1\}
\]

Finally, conditional on $K=k$, choose $k+1$ values $D_i$
(for $i=1 \dots k+1$) \iid from $U(0,1)$. This generates a random
function $f$:

\[
f(x)=\sum_{i=1}^{k+1} \1{x \in I_{i}} D_i
\]

As a default, take $\alpha=\frac{1}{2}$.

This prior is related to the prior described in Diaconis and
Freedman~\cite{df2}, but this prior differs in that position of the
split points is random. It is similar, however, in that it specifies a
prior on piecewise constant functions. 




\section{The Posterior}

Figure~\ref{f:post1} shows an example of the posterior mean of this
prior upon seeing $16,384$ points randomly labeled according to the
function $f$ described in section~\ref{s:example}. The solid grey
curve is the true $f$, as before. The solid black curve is the result
of running $30,000$ MCMC iterations following the general procedures
described in M{\o}ller~\cite{moller}.

To give some sense of how well we
are doing, a very na\:ive ``frequentist'' estimate is
superimposed. Specifically, the unit interval is divided into $20$
equally spaced segments. For each segment, all the data lying within
the segment is considered giving $k_0$ 0's and $k_1$ 1's within the
segment. Each segment is then labeled with three horizontal bars. The
middle bar is the sample mean on that segment
(i.e. $\hat{d}=k_1/(k_0+k_1)$). The upper and lower bars give a na\:ive
95\%-confidence interval for the value there via $\hat{d} \pm
2\sqrt{\hat{d}(1-\hat{d})/(k_0+k_1)}$. We can see that there is still
plenty of noise left in the data, despite its apparent abundance.

Roughly speaking, the posterior mean seems to be doing a good job of
finding the split points between the piecewise constant regions. It
manages to approximate the continuously varying region fairly well,
but detects little deviation from constancy on the two constant intervals.

\section{Computing the Posterior}

Computation of the posterior is simplified by identifying the
posterior distribution of the $(k+1)$ values $D_i$. If we
condition on $K=k$ and on the location of the split points then, a
priori, $D_i$ are independent $U(0,1)$. A posteriori, they are
(conditionally) independent and beta distributed with parameters:
\begin{align*}
a_i&=(\textrm{\# of data points in $I_i$ labeled 1})+1 \\
b_i&=(\textrm{\# of data points in $I_i$ labeled 0})+1.
\end{align*}

Using this fact, we can integrate out the $D$'s from our
posterior (i.e. we do not have to explicitly simulate realizations of
the $D$'s since this completely describes their (conditional)
posterior distribution).

All that remains, then, is to perform a random walk over the point
process with $K=k$ points $C_1, \dots, C_k$. Our posterior weight on a
particular choice $K=k$ and $\Cvec=\cvec$ (treating the $C$'s as a random
vector) is proportional to the prior
probability times the predictive probability of the data (having
integrated out the $D$'s).

Specifically, if we denote the predictive probability of the data under $K=k$ and
$\Cvec=\cvec$ by:
\[
\psi(k, \cvec)=\prod_{i=1}^{k+1} \textrm{beta integral}(a_i,b_i)
\]

and the density of the prior (with respect to a poisson point process
with parameter $\lambda=1$) as:

\[
\pi(k,\cvec)=@@.
\]

Then our posterior has density proportional to:
\[
\pi(k,\cvec)\psi(k, \cvec).
\]

To sample from this posterior, we make proposals according to a base
chain, and accept the proposals according to the Metropolis-Hastings
algorithm. Our base chain proposes one of 6 actions at each step
randomly with probability:
\begin{verbatim}
 1         2         3         4         5         6
 0.0476    0.0476    0.2381    0.1429    0.4762    0.0476
\end{verbatim}

Action 1 adds a new coordinate chosen uniformly on [0,1]. Action 2
deletes a coordinate at random. Action 3 chooses a random coordinate
and moves it by a small random normal amount (standard deviation 0.1)
(no action taken if the move is invalid). Action 4 chooses a random
coordinate and moves it to a new value chosen uniformly from
[0,1]. Action 5 moves all coordinates by a very small random normal
amount (standard deviation 0.01) (a coordinate doesn't move if this would
propose a move outside the interval, but all valid moves are still
taken). Action 6 re-randomizes all the coordinates with uniform values
from [0,1].

\begin{figure}
\noindent
\begin{minipage}[t]{\linewidth}
  \centering%\epsfig{figure=../unifpost_N16384_05_1.ps,height=7cm,angle=90}
  \caption[]{Posterior Mean et.al.}\label{f:post1}
\end{minipage}
\end{figure}

 A selection of popular algorithms includes: nearest
neighbors, local regression (e.g. kernel methods and loess-type
algorithms), ``global'' regressions (e.g. neural nets and support
vector machines), and partition based (e.g. CART). (bagging/boosting?)
Most of these methods can be described (at least in principle) as
specifying a certain class of functions (either locally or globally)
and choosing among the candidates by optimizing some criterion which
is intended to balance the ever-important tradeoff between fidelity to
the data and the possibility of ``over-fitting.'' There are at least
three different competing ``philosophies'' for how exactly such
criteria should be chosen. Traditional frequentists tend to evaluate
criteria in terms of ``bias/variance tradeoffs.''  Typically, they
propose criteria which utilize theoretically motivated point estimates
of risk (e.g. $C_p$, GCV, and cross-validation). Advocates of
``Structural Risk Minimization,'' on the other hand, penalize a
function according to the complexity of the function class that
contains it (according to a pre-decided ``structure'') in order to
maintain upper-confidence levels on the risk. A purely Bayesian
approach, however, would be to specify whatever subjective prior the
practitioner happens to believe, and choose the estimate which
minimizes \emph{posterior} risk.

Each approach has its advantages and disadvantages. The frequentist
approach has the
most direct information about the (asymptotic) sampling variation of its estimates
(under a fixed truth). Little, however, can typically be said about
the finite sample properties of its estimates for general $F$. Structural Risk Minimization offers
theoretically sound confidence statements about its particular risk on
a particular data set, under sampling from an arbitrarily complicated
$F$. It does not, however, have anything to say about the
finite-sample optimality of its estimation scheme under any
particular (prior) scenario--this is especially true if one considers
a scenario in which arbitrary $F$ may be possible,
but are vanishingly unlikely. A subjective Bayesian approach offers
the fact that it is behaving optimally for at least some scenario (the
one specified by its prior). It typically, however, shows little concern for
its sampling variation (under particular $F$), or interest in offering uniformly valid confidence statements about its risk.

It is the opinion of this paper that the best chance of attaining all
of the advantages outlined above is to employ the Bayesian approach,
but carefully choose the prior to satisfy both of the ``empiricist'' goals.

\begin{thebibliography}{1}
\bibitem{df1}
P. Diaconis and D. Freedman (1986). On the Consistency of Bayes Estimates. \emph{Ann. Stat.} \textbf{14}, 1-26
\bibitem{df2}
P. Diaconis and D. Freedman (1990). On the Uniform Consistency of Bayes Estimates for Multinomial Probabilities. \emph{Ann. Stat.} \textbf{18}, 1317-1327
\bibitem{df3}
P. Diaconis and D. Freedman (1993). Nonparametric Binary Regression: A
Bayesian Approach. \emph{Ann. Stat.} \textbf{21}, 2108-2137
\bibitem{moller}
J. M{\o}ller (1999). Stochastic Geometry: Likelihood and Computation
(chapter 4). O.~Barndorff-Nielsen, W.~Kendall, and M.~van~Lieshout,
eds. Chapman and Hall.
\bibitem{mollerskare}
J. M{\o}ller and {\O}ivind Skare (??) Bayesian Image Analysis with Coloured Voronoi Tessellations and a View to Application in Reservoir Modelling
\end{thebibliography}

We
also define the function:
\[
\tilde{f_0}(x,y)=f_0(x)\1{y=1}+(1-f_0(x))\1{y=0}
\]
and when it does not result in confusion we drop the tilde.

